Source Code Comments: Overlooked in the Realm of Code Clone Detection

Reusing code can produce duplicate or near-duplicate code clones in code repositories. Current code clone detection techniques, like Program Dependence Graphs, rely on code structure and their dependencies to detect clones. These techniques are expensive, using large amounts of processing power, time, and memory. In practice, programmers often utilize code comments to comprehend and reuse code, as comments carry important domain knowledge. But current code detection techniques ignore code comments, mainly due to the ambiguity of the English language. Recent advances in information retrieval techniques may have the potential to utilize code comments for clone detection. We investigated this by empirically comparing the accuracy of detecting clones with solely comments versus solely source code (without comments) on the JHotDraw package, which contains 315 classes and 27K lines of code. To detect clones at the file level, we used a topic modeling technique, Latent Dirichlet Allocation, to analyze code comments and GRAPLE -- utilizing Program Dependency Graph -- to analyze code. Our results show 94.86 recall and 84.21 precision with Latent Dirichlet Allocation and 28.7 recall and 55.39 precision using GRAPLE. We found Latent Dirichlet Allocation generated false positives in cases where programs lacked quality comments. But this limitation can be addressed by using a hybrid approach: utilizing code comments at the file level to reduce the clone set and then using Program Dependency Graph-based techniques at the method level to detect precise clones. Our further analysis across Java and Python packages, Java Swing and PyGUI, found a recall of 74.86\% and a precision of 84.21\%. Our findings call for reexamining the assumptions regarding the use of code comments in current clone detection techniques.

==> abstract.tex <==
\begin{abstract}
\label{sec:abstract}
What is problem?
 Reusing code can produce duplicate or near-duplicate code clones in code repositories. Current code clone detection techniques, like Program Dependence Graphs (PDGs), depend on code structure and their dependencies to detect clones. These techniques are expensive, using large amounts of processing power, time, and memory. In practice, programmers often utilize code comments to understand, comprehend, and
reuse code, as comments carry important domain knowledge.
But current code detection techniques ignore code comments, mainly due to the ambiguity of English language. Recent advances in information retrieval techniques may have the potential to utilize code comments for clone detection. We investigated the possibility of this use of code comments by empirically comparing the accuracy of detecting clones with solely code versus solely comments on a JHotDraw package, which contains 315 classes and 25KLOC. To detect clones at the file level, we used a topic modeling technique, Latent Dirichlet Allocation (LDA) to analyze code comments and GRAPLE -- utilizing Program Dependency Graph (PDG) -- to analyze code. Our results show 94.86\% recall and 84.21\% precision  with LDA and 28.7\% recall and 55.39\% precision using GRAPLE. We found lack of quality comments can generate large number of false positives. But this can be addressed by using a hybrid approach: utilizing code comments at the file level to reduce the clone set and then using PDG based techniques to detect precise clones at the method level. Our further analysis across Java and Python packages, Java Swing and PyGUI found recall of 74.86.68\% and precision of 84.21\%. Our findings call for reexamining the assumption regarding code comments with current clone detection techniques.




Reusing code  can produce duplicate or near-duplicate code clones in code repositories. Current code clone detection techniques, like Program Dependence Graphs (PDGs), depend on code structure and their dependencies to detect clones and are expensive and resource-intensive. From a program comprehension point of view, programmers often use code comments to understand and reuse code, as they carry important domain information; but code comments are ignored by current code detection techniques. This paper investigates the use of code comments for clone detection by  empirically comparing the accuracy of detecting clones with solely code versus solely comments on a JHotDraw package, which contains 315 classes and 25KLOC. To detect clones at the file level, we used a topic modeling technique, Latent Dirichlet Allocation (LDA) to analyze code comments and Program Dependency Graph (PDG) to analyze code. Our results show 94.86\% recall and 84.21\% precision  with LDA and 28.7\% recall and 55.39\% precision using GRAPLE.  Our  further analysis across Java and Python packages found recall of 90.68\% and precision of 49.49\% for Java Swing (318 source files with 30KLOC); and recall of 51.12\%  and precision of 39.21\%  PyGUI (355 source files with 28KLOC). We found that better quality comments can help in detecting clones by LDA and using a hybrid approach, utilizing code comments at file level to narrow the number of clones and using PDG to detect clones at method and statement level. Our findings call for reexamining the assumption regarding clone detection techniques.



Reusing code can produce duplicate or near-duplicate code clones in code repositories. The current code clone detection techniques like Program Dependence Graphs (PDGs), depends on code structure and their dependencies to detect clones and are expensive and resource-intensive.From program comprehension point of view, programmers often use code comments to understand and reuse code as they carry important domain information; but code comments are ignored by current code detection techniques.This paper investigates the realm of code comments for clone detection by  empirically comparing the accuracy of detecting clones with just code or just comments on a JHotDraw package, which contains 310 classes. To detect clones at file level, we used a topic modeling technique, Latent Dirichlet Allocation to analyze code comments and Program Dependency Graph (PDG) to analyze code. Our results show 84.21\% precision and 94.86\% recall with LDA and 55.39\% precision and 28.7\% recall using GRAPLE.  Our  further analysis across Java and Python packages found recall of 90.68\% and precision of 49.49\% for Java Swing (318 java source files with 30KLOC); and recall of 51.12\%  and precision of 39.21\%  PyGUI (355 java source files with 28KLOC). We found that better quality comments can help in detecting clones by LDA and using a hybrid approach utilizing code comments at file level to narrow the number of clones and using PDG to detect clones at method and statement level. Our findings call for the attention to reexamine the assumption regarding clone detection.

 

% From a program comprehension point of view, comments carry important domain knowledge and can assist in program understanding. However, comments have been widely ignored by most of the clone detection techniques. We strive to empirically evaluate the clone detection mechanisms using both code and comments on JHotDraw package, JFreeChart, JavaNIO, and Java Swing. Our results for JHotDraw using LDA indicates a precision of 84.21\% and a recall of 74.86\% which is much higher compared to GRAPLE with precision and recall of 55.39\% 28.7\%, respectively. To uphold our hypothesis, we further compared and contrasted the clone sets generated by LDA and GRAPLE (PDG-Based) for all the java packages. In the end, to extend our logic over the cross-language domain, we analyzed two packages of same functionality but of different languages, PyGUI and Java Swing. The results proponents that comments can be used to find semantic clones. Thus, it necessitates a need to reexamine the assumptions regarding semantic clone detection techniques.


% From a program comprehension point of view, comments carry important domain knowledge and can assist in program understanding. However, comments have been ignored by most of the clone detection techniques. We empirically evaluated the detection mechanisms using both code and comments on JHotDraw package, JFreeChart, JavaNIO, and Java Swing. Our results for JHotDraw using LDA indicates a precision of 84.21\% and a recall of 74.86\% which is much higher compared to GRAPLE (PDG-based). We also compared and contrasted the clone sets generated by LDA and GRAPLE for the java packages. The cross-language clone detection was obtained between PyGUI (python package) and Java Swing. The results proponents that comments can be used to find semantic clones. Thus, it necessitates a need to reexamine the assumptions regarding semantic clone detection techniques.

% Programmers reuse code to increase their productivity, which leads to large fragments of duplicate or near-duplicate code in the code base. The current code clone detection techniques for finding semantic clones utilize Program Dependence Graphs (PDG), which are expensive and resource-intensive.

% Programmers reuse code to increase their productivity, which leads to large fragments of duplicate or near-duplicate code in the code base. The current code clone detection techniques for finding semantic clones utilize Program Dependence Graphs (PDG), which are expensive and resource-intensive. Program Dependence Graphs and other clone detection techniques utilize code and have completely ignored the comments. From a program comprehension point of view, comments carry important domain knowledge and assist in program understanding. Hence, a major part of the program is ignored while detecting clones. This paper investigates the realm of comments for clone detection. We empirically evaluated the accuracy of detecting clones with both code and comments on a JHotDraw package, which contains 310 classes. Our results show that detecting code clones in the presence of comments, using the natural language processing tool, Latent Dirichlet Allocation, gave 84\% precision and 94\% recall. While in the presence of a Program Dependence Graph, using GRAPLE, we got 55\% precision and 29\% recall. These results indicate that comments can be used to find  semantic clones. We recommend  utilizing comments with Latent Dirichlet Allocation (LDA) to find clones at the file level and code with PDG for finding clones at the function level. These findings necessitate a need to reexamine the assumptions regarding semantic clone detection techniques.


% Programmers reuse code to increase their productivity, which leads to large fragments of duplicate or near-duplicate code in the code base. The current code clone detection techniques for finding semantic clones utilize Program Dependence Graphs (PDG), which are expensive and resource-intensive. Program Dependence Graphs and other clone detection techniques utilize code and have completely ignored the comments. From a program comprehension point of view, comments carry important domain knowledge and assist in program understanding. Hence, a major part of the program is ignored while detecting clones. This paper investigates the realm of comments for clone detection. We empirically evaluated the accuracy of detecting clones with both code and comments on a JHotDraw package, which contains 310 source files. Then we compared and contrasted the clone sets generated by LDA for JFreeChart (1015 source files) and Java NIO (154 source files). Our last step, was to use LDA To detect clones in cross-language, Java and Python. Our results show that detecting code clones in the presence of comments, using the natural language processing tool, Latent Dirichlet Allocation, gave 84.21\% precision and 94.86\% recall in case of JHotDraw while in the presence of a Program Dependence Graph, using GRAPLE, we got 55\% precision and 29\% recall. Interestingly, LDA always generate a much higher number of clone sets compared to PDG. Similarly, for our cross language anlysis we received a precision of 84.21\% and a recall of 74.86\%.  These results indicate that comments can be used to find  semantic clones. We recommend  utilizing comments with Latent Dirichlet Allocation (LDA) to find clones at the file level and code with PDG for finding clones at the function level. These findings necessitate a need to reexamine the assumptions regarding semantic clone detection techniques.

\end{abstract}

==> bib.tex <==

\begin{thebibliography}{00}

\bibitem{akash2018} A. Ghosh and S. K. Kuttal, Semantic Code Clones: Can Source Code Comments Help?, IEEE Conference VL/HCC, 2018.

\bibitem{Sdang} S. Dang and S. A. Wani, Performance Evaluation of Clone Detection Tools, International Journal of Science and Research, 2015

\bibitem{quality} C. K. Roy, J. R. Cordy, and R. Koschke, Comparison and evaluation of code clone detection techniques and tools: A qualitative approach, Science of Computer Programming, 74(7), 2009.

\bibitem{survey} A. Sheneamer and J. Kalita, Article: A Survey of Software Clone Detection Techniques, International Journal of Computer Applications, 137(10) 2016.

\bibitem{duplicate} M. Sudhamani and L. Rangarajan, Duplicate Code Detection using Control Statements, International Journal of Computer Applications Technology and Research, 4(10), 2015

\bibitem{KTStolee} K. T. Stolee, S. Elbaum, and Daniel Dobos, Solving the Search
for Source Code, ACM Transactions on Software Engineering Methodology, 23(3), pp.26, 2014

\bibitem{rafhoff} R. Hoffmann, J. Fogarty, and D. S. Weld, Assieme: finding and leveraging implicit references in a web search interface for programmers, In
Proceedings of the 20th annual ACM symposium on User interface software and
technology, pp.13–22, 2007.

\bibitem{dejavu} Lopes, Cristina V., Petr Maj, Pedro Martins, Vaibhav Saini, Di Yang, Jakub Zitny, Hitesh Sajnani, and Jan Vitek, DéjàVu: a map of code duplicates on GitHub, In Proceedings of the ACM on Programming Languages 1, OOPSLA, pp.84, 2017


\bibitem{avetisyan} A. Avetisyan, S. Kurmangaleev, S. Sargsyan, M. Arutunian,
and A. Belevantsev. LLVM-based code clone detection framework. Computer Science and Information Technologies, pp.100-104, 2015.

\bibitem{clcminer} X. Cheng, Z. Peng, L. Jiang, H. Zhong, H. Yu, and J. Zhao, CLCMiner: Detecting Cross-Language Clones without Intermediates. IEICE Trans, on Information and Systems, 100(2), pp.273-284, 2017.

\bibitem{Sirres} R. Sirres, T. F. Bissyandé, D. Kim, D. Lo, J. Klein,
K. Kim, and Y. L. Traon, Augmenting and Structuring User Queries to Support Efficient Free-Form Code Search, In Proceedings of Empirical Software Engineering, 23(5), pp.2622–2654, 2018.

\bibitem{kraft} N. A. Kraft, B. W. Bonds, and R. K. Smith, Cross-language Clone Detection, In Proceedings of SEKE, pp.54-59, 2008.

\bibitem{white} M. White, M. Tufano,C.Vendome, and D. Poshyvanyk, Deep learning code fragments for code clone detection, In Proceedings of the 31st IEEE/ACM International Conference on Automated Software Engineering, pp.87-98, 2016

\bibitem{Facoy2018} K. Kim, D. Kim, TF Bissyande, E. Choi, L.li, J. Klein, Y. Le Traon,  FaCoY–A Code-to-Code Search Engine, In Proceedings of the 40th International Conference on Software Engineering, 2018

\bibitem{LICCA2018} T. Vislavski, G. Rakic, Z and N Budimac, LICCA: A tool for cross-language clone detection, 2018 IEEE 25th International Conference on Software Analysis, Evolution and Reengineering, pp.512-516, 2018


\bibitem{Higo2011} Y. Higo, U. Yasushi, M. Nishino, and S. Kusumoto, Incremental code clone detection: A PDG-based approach, In Proceedings of Working Conference on Reverse Engineering, pp.3-12, 2011

\bibitem{Higo2009} Y. Higo and S. Kusumoto, Enhancing quality of code clone detection with program dependency graph, In Proceedings of Working Conference on Reverse Engineering, pp.315-316, 2009.

 \bibitem{JHD} JHotDraw: http://www.jhotdraw.org/

\bibitem{PYGUI} PyGUI: http://www.cosc.canterbury.ac.nz/greg.ewing/pythongui/version/
Doc/index.html

\bibitem{JAVASwing} 
Java Swing: https://docs.oracle.com/javase/javax/swing/package-summary.html

\bibitem{jfree} JFreeChart: http://www.jfree.org/jfreechart/

\bibitem{nio} Java NIO: https://docs.oracle.com/javase/7/docs/api/index.html?java/nio/
file/package-summary.html

\bibitem{exp} https://docs.python.org/3/tutorial/errors.html

\bibitem{Basit} H. Basit, D. Rajapakse, and S. Jarzabek, An empirical study on limits of clone unification using generics, In Proceedings of SEKE, pp.109-114, 2005.

\bibitem{Girish} G. Maskeri, S Sarkar and K Heafield, Mining business topics in source code using latent dirichlet allocation, In Proceedings of 1st India software engineering conference, pp.113-120, 2008.

\bibitem{LDA} D. Blei, A. Ng, and M. Jordan, Latent dirichlet allocation, Journal of Machine Learning Research, pp.993-1022, 2003.

\bibitem{Griffiths} T. Griffiths and M. Steyvers, Finding scientific topics, In Proceedings of the National Academy of Sciences, pp.5228-5235, 2004.

\bibitem{Nakakoji} K. Nakakoji, Y. Yamamoto, Y. Nishinaka, Kouichi Kishida, and Y. Ye, Evolution Patterns of Open-Source Software Systems and Communities, In Proceedings of the International Workshop on Principles of Software Evolution, pp.76-85, 2002.

\bibitem{Gu2016} Xiaodong Gu, Hongyu Zhang, Dongmei Zhang, and Sunghun Kim. 2016. Deep
API learning. In Proceedings of the 2016 24th ACM SIGSOFT International Symposium on Foundations of Software Engineering. ACM, 631–642.

\bibitem{Haiduc2010a} Sonia Haiduc, Jairo Aponte, and Andrian Marcus. 2010. Supporting program
comprehension with source code summarization. In Proceedings of the 32nd
ACM/IEEE International Conference on Software Engineering-Volume 2. ACM, 223–
226.
\bibitem{Haiduc2010b} Sonia Haiduc, Jairo Aponte, Laura Moreno, and Andrian Marcus. 2010. On the
use of automated text summarization techniques for summarizing source code.
In Reverse Engineering (WCRE), 2010 17th Working Conference on. IEEE, 35–44.

%\bibitem{Sridhara2010} Giriprasad Sridhara, Emily Hill, Divya Muppaneni, Lori Pollock, and K VijayShanker. 2010. Towards automatically generating summary comments for java methods. In Proceedings of the IEEE/ACM international conference on Automated software engineering. ACM, 43–52.

\bibitem{Iyer2016} Srinivasan Iyer, Ioannis Konstas, Alvin Cheung, and Luke Zettlemoyer. 2016.
Summarizing Source Code using a Neural Attention Model.. In ACL (1).

\bibitem{Loyola2017} Pablo Loyola, Edison Marrese-Taylor, and Yutaka Matsuo. 2017. A Neural Architecture for Generating Natural Language Descriptions from Source Code
Changes. arXiv preprint arXiv:1704.04856 (2017).

\bibitem{McBurney2014} Paul W McBurney and Collin McMillan. 2014. Automatic documentation generation via source code summarization of method context. In Proceedings of the
22nd International Conference on Program Comprehension. ACM, 279–290.

\bibitem{Moreno2013} Laura Moreno, Jairo Aponte, Giriprasad Sridhara, Andrian Marcus, Lori Pollock,
and K Vijay-Shanker. 2013. Automatic generation of natural language summaries
for java classes. In Program Comprehension (ICPC), 2013 IEEE 21st International Conference on. IEEE, 23–32.

\bibitem{Sridhara2010} Giriprasad Sridhara, Emily Hill, Divya Muppaneni, Lori Pollock, and K VijayShanker. 2010. Towards automatically generating summary comments for java
methods. In Proceedings of the IEEE/ACM international conference on Automated
software engineering. ACM, 43–52.

\bibitem{Wang2016} Song Wang, Taiyue Liu, and Lin Tan. 2016. Automatically learning semantic
features for defect prediction. In Proceedings of the 38th International Conference
on Software Engineering. ACM, 297–308.

\bibitem{White2016} Martin White, Michele Tufano, Christopher Vendome, and Denys Poshyvanyk.
2016. Deep learning code fragments for code clone detection. In Proceedings of
the 31st IEEE/ACM International Conference on Automated Software Engineering.
ACM, 87–98.

\bibitem{hu2018} Xing Hu, Ge Li, Xin Xia, David Lo, and Zhi Jin. 2018. Deep code comment generation. In Proceedings of the 26th Conference on Program Comprehension, 200-210.

\bibitem{MCIdiff} Y. Lin, Z. Xing, Y. Xue, Y. Liu, X. Peng, J. Sun, and W. Zhao, Detecting differences across multiple instances of code clones, In Proceedings of International Conference on Software Engineering, pp.164-174, 2014.

\bibitem{nicad} J.R. Cordy and C. K. Roy, The NiCad clone detector, In Proceedings of Program Comprehension (ICPC), pp.219-220, 2011.

\bibitem{CloneDR}I.D. Baxter, A. Quigley, L. Bier, M. Sant’Anna, L. Moura, and A. Yahin, CloneDR: clone detection and removal, In Proceedings of the 1st International Workshop on Soft Computing Applied to Software Engineering, pp.111-117, 1999.

\bibitem{Howard1994} J. Howard Johnson, Visualizing textual redundancy in legacy source, In Proceedings of the conference of the Centre for Advanced Studies on Collaborative research, John Botsford, Ann Gawman, Morven Gentleman, Evelyn Kidd, Kelly Lyons, Jacob Slonim, and Howard Johnson (Eds.). IBM Press, 1994.

\bibitem{Cheng} H. Cheng, X. Yan, and J. Han, Mining Graph Patterns, In Frequent Pattern Mining, pp.307-338, 2014.

\bibitem{Biggerstaff} T. J. Biggerstaff, B. G. Mitbander, and D. Webster, Program understanding and the concept assignment problem, Communications of the ACM, 37(5):pp.72-83, 1994.

\bibitem{Caprile} B. Caprile and P. Tonella, Nomen est omen: Analyzing the language of function identifiers, In Proceedings of the Sixth Working Conference on Reverse Engineering, pp.112-122, 1999.

\bibitem{Anquetil} N. Anquetil and T. C. Lethbridge, Recovering software architecture from the names of source files, Journal of Software Maintenance: Research and Practice, 11(3),pp.201-221, 1999.

\bibitem{Wilde} N. Wilde, M. Buckellew, H. Page, V. Rajlich, and L. Pounds, A comparison of methods for locating features in legacy software, Journal of Systems and Software, 65(2), pp.105-114, 2003.

\bibitem{Kuhn} A. Kuhn, S. Ducasse, and T. Gˆırba, Semantic clustering: Identifying topics in source code, Information and Software Technology, 49(3), 2006. 

\bibitem{Antoniol 2012} G. Antoniol, G. Canfora, G. Casazza, A. De Lucia and E. Merlo, Recovering traceability links between code and documentation, In Proceedings of IEEE Transactions on Software Engineering, 28(10), pp.970-983, 2002.

\bibitem{Krinke} J. Krinke, Identifying similar code with program dependence graphs. In Proceedings of Working Conference on Reverse Engineering, pp.301-309, 2001. 

\bibitem{Komondoor} R. Komondoor and S. Horwitz, Using Slicing to Identify Duplication in Source Code, In Proceedings of International static analysis symposium, pp.40-56, 2001.

\bibitem{Higo} Y. Higo and S. Kusumoto, Code Clone Detection on Specialized PDGs with Heuristics, In Proceedings of Software Maintenance and Reengineering, pp.75-84,  2011.

\bibitem{Pham} N. H. Pham, H. A. Nguyen, T. T. Nguyen, J. M. Al-Kofahi, and T. N. Nguyen, Complete and accurate clone detection in graph-based models, In Proceedings of International Conference on Software Engineering, pp.276-286, 2009

\bibitem{Tenny} T. Tenny, Program Readability: Procedures Versus Comments, IEEE Transactions of Software Engineering, 14(9), pp.1271-1279, 1988.

\bibitem{Woodfield} S. N. Woodfield, H. E. Dunsmore, and V. Y. Shen, The effect of modularization and comments on program comprehension, In Proceedings of International Conference on Software Engineering, pp.215-223, 1981.

\bibitem{Souza} S. C. B. de Souza, N. Anquetil, and K. M. de Oliveira, A Study of the Documentation Essential to Software Maintenance, In Proceedings of the 23rd annual international conference on Design of communication: documenting \& designing for pervasive information, pp.68-75, 2005.

\bibitem{Ferrante}J. Ferrante, K. J. Ottenstein, and J. D. Warren, The program dependence graph and its use in optimization, ACM Transactions on Programming Languages and Systems, 9(3), pp.319-349, 1987.

\bibitem{Baker1995} B. Baker, On Finding Duplication and Near-Duplication in Large Software Systems, In Proceedings of Working Conference on Reverse Engineering, pp. 86-95, 1995.

\bibitem{Baxter1998} I. Baxter, A. Yahin, L. Moura and M. Anna, Clone Detection Using Abstract Syntax Trees, In Proceedings of Software Maintenance, pp.368-377, 1998.

\bibitem{Kapser2006} C. Kapser and M. Godfrey, Supporting the Analysis of Clones in Software Systems: A Case Study. Journal of Software Maintenance and Evolution: Research and Practice , 18(2), pp.61-82, 2006.

\bibitem{Mayrand1996} J. Mayrand, C. Leblanc and E. Merlo, Experiment on the Automatic Detection of Function Clones in a Software System Using Metrics, In Proceeding of ICSM, pp.244-253, 1996Measuring Code Behavioral Similarity for Programming and Software Engineering
Education.

\bibitem{shihan} S. Li, X. Xiao, B. Bassett, T. Xie, and Nikolai Tillmann, Measuring Code Behavioral Similarity for Programming and Software Engineering
Education, In Proceedings of the 38th International Conference on Software
Engineering Companion, pp.501–510, 2016.

\bibitem{kim} H. Kim, Y. Jung, S. Kim, and K. Yi, MeCC: Memory comparison-based
clone detector, In Proceedings of the 33rd International Conference on Software
Engineering, pp.301–310, 2011.


\bibitem{fhsu} F. H. Su, J. Bell, K. Harvey, S. Sethumadhavan, G.
Kaiser, and T. Jebara, Code Relatives: Detecting Similarly Behaving
Software, In Proceedings of the 2016 24th ACM SIGSOFT International Symposium
on Foundations of Software Engineering (FSE 2016), pp.702–714, 2016.

\bibitem{Al-Omari2012}	F. Al-Omari, I. Keivanloo, C. K. Roy, and J. Rilling, Detecting clones across microsoft .net programming languages, In Proceedings of Working Conference on Reverse Engineering, pp.405-414, 2012. 	

\bibitem{Bazrafshan}S. Bazrafshan, and R. Koschke, An empirical study of clone removals, In Proceedings of International Conference Software Maintenance, pp.50-59, 2013.

\bibitem{Lxiang} L. Jiang and Z. Su, Automatic mining of functionally equivalent
code fragments via random testing. In Proceedings of the eighteenth international
symposium on Software testing and analysis, pp.81–92, 2009.

\bibitem{Asaduzzaman2012} M. Asaduzzaman, C. K. Roy, and K. A. Schneider, VisCad: Flexible code clone analysis support for NiCad, In Proceedings of International Workshop on Software Clones, pp.77-78, 2011.

\bibitem{Baxter} I. Baxter, A. Yahin, L. Moura, M. Sant’Anna, and L. Bier, Clone detection using abstract syntax trees, In Proceedings of International Conference on Software Maintenance, pp.368-377, 1998.	

\bibitem{Bellon} S. Bellon, R. Koschke, G. Antoniol, J. Krinke, and E. Merlo, Comparison and evaluation of clone detection tools, IEEE Transaction on Software Engineering, 33(9), pp.577-591, 2007.

\bibitem{Bettenburg} N. Bettenburg, W. Shang, W. Ibrahim, B. Adams, Y. Zou, and A. Hassan, An empirical study on inconsistent changes to code clones at the release level, Science of Computer Programming, 77(6), pp.760-776, 2012.

\bibitem{Bouktif} S. Bouktif, G. Antoniol, M. Neteler, and E. Merlo, A novel approach to optimize clone refactoring activity, In Proceedings of Genetic and Evolutionary Computation, pp.1885-1892, 2006.

\bibitem{Adar}	E. Adar and M. Kim, SoftGUESS: Visualization and exploration of code clones in context, In Proceedings of International Conference on Software Engineering, pp.762-766, 2007.

\bibitem{Chatterji}	D. Chatterji, J. C. Carver, and N. A. Kraft, Cloning: The need to understand developer intent, In Proceedings of International Workshop on Software Clones, pp.14-15, 2013.

\bibitem{Cordy2003}	J. R. Cordy. Comprehending reality: Practical barriers to industrial adoption of software maintenance automation, In Proceedings of International Workshop on Program Comprehension, pp.196-206, 2003.

\bibitem{Cordy2011}	J. R. Cordy, Live scatterplots, In Proceedings of International Workshop on Software Clones, pp.79-80, 2011.

\bibitem{Gode} N. Göde, and K. Rainer, Studying clone evolution using incremental clone detection,  Journal of Software: Evolution and Process, 25(2), pp.165-192, 2013.

\bibitem{Grinstead} C. M. Grinstead and J. L. Snell, Introduction to Probability, American Mathematical Society, Providence, RI, 2 edition, 1997.

\bibitem{Roy2014} C.K. Roy, M.F. Zibran, and R. Koschke, The vision of software clone management: Past, present, and future (Keynote paper), In Proceedings of IEEE Software Maintenance, Reengineering and Reverse Engineering, pp.18-33, 2014.

\bibitem{Henderson} TAD Henderson and A Podgurski, Sampling code clones from program dependence graphs with GRAPLE, In Proceedings of the 2nd International Workshop on Software Analytics, pp.47-53, 2016.

\bibitem{Gabel} M. Gabel, L Jiang, Zhendong SU, Scalable detection of semantic clones, In Proceedings of the International Conference on Software Engineering, pp.321-330, 2008.

\bibitem{Roy2007} C. K. Roy and J. R. Cordy, A survey on software clone detection research, Technical Report TR 2007-541, Queens University, 2007.

\bibitem{Thompson} S. K. Thompson. Sampling. John Wiley and Sons, New York, 2 edition, 2002.

\bibitem{Johnson}J. Johnson, Visualizing Textual Redundancy in Legacy Source, In Proceedings of CASCON, pp.171-183, 1994.

\bibitem{Seidl} D. Seidl, B. Hummel and E. Juergens, Quality Analysis of Source Code comments, In Proceedings of International Conference on Program Comprehension, pp.43-60, 2013.

\bibitem{Oezbek} C. Oezbek and L. Prechelt, JTourBus: Simplifying Program Understanding by Documentation that Provides Tours Through the Source Code, In Proceedings of IEEE International Conference on Software Maintenance, pp.64-73, 2007.

\bibitem{Podgurski} G. Shu, B.Sun, T.A.D. Henderson and A. Podgurski, JavaPDG: A New Platform for Program Dependence Analysis, In Proceedings of International Conference on Software Testing, Verification and Validation, pp.408-415, 2013.

\bibitem{Higo13} Yoshiki Higo and Hiroaki Murakami and Shinji Kusumoto, Revisiting Capability of PDG-based Clone Detection, Technical Report, Graduate School of Information Science and Technology, Osaka University, 2013.

\bibitem{Al-Omari} F. Al-Omari, I. Keivanloo, C. K. Roy, and J. Rilling, Detecting clones across Microsoft .net programming languages, In Proceeding of Working Conference on Reverse Engineering, pp.405-414, 2012.

\bibitem{Keivanloo} I. Keivanloo, C. K. Roy, and J. Rilling, SeByte: Scalable clone and similarity search for bytecode, Science of Computer Programming, 95, 2014
					
\bibitem{Davis} I. Davis and M. Godfrey, Clone detection by exploiting assembler, In Proceedings of 4th International Workshop on Software Clones, pp.77-78, 2010.

\end{thebibliography}

==> biblog.tex <==
\begin{thebibliography}{00}

\bibitem{reuse1} T. C. Jones (1986). Programming Productivity. McGraw-Hill.
\bibitem{reuse2} C. W. Krueger (1992). "Software reuse". In ACM Computing Surveys. 24(2):131-183.
\bibitem{reuse3} V. Basili (1990). Viewing maintenance as reuse-oriented software development. In IEEE Software, 7(1):19–25, Jan.

\bibitem{reuse4} V. Basili and H. D. Rombach (1991). "Support for comprehensive reuse". In IEE Software Engineering Journal. Sept. pp. 303-316

\bibitem{reuse5} H. D. Rombach (1991). Software reuse: a key to the maintenance problem. In Information and Software Technology Journal, 33(1), Jan/Feb.

\bibitem{reuse6} Hubig R., Morschel I. (1997) Quality and Productivity Improvement in Object-Oriented Software Development. In: Lehner F., Dumke R., Abran A. (eds) Software Metrics. Information Engineering und IV-Controlling. Deutscher Universitätsverlag, Wiesbaden

\bibitem{reuse7} Charles W. Krueger. 1992. Software reuse. ACM Comput. Surv. 24, 2 (June 1992), 131–183.


\bibitem{comment1} T. Tenny, “Program Readability: Procedures Versus Comments,” IEEE Trans. Softw. Eng., vol. 14, no. 9, 1988.
 

\bibitem{comment2} S. N. Woodfield, H. E. Dunsmore, and V. Y. Shen, “The effect of modularization and comments on program comprehension,” ser. ICSE’81, 1981.
 

\bibitem{comment3} S. C. B. de Souza, N. Anquetil, and K. M. de Oliveira, “A Study of the Documentation Essential to Software Maintenance,” ser. SIGDOC ’05, 2005.

\bibitem{popular}  Popular  Programming  Language  (2020).URL  https://www.tiobe.com/tiobe\-index/

\bibitem{Adar}	E. Adar and M. Kim, SoftGUESS: Visualization and exploration of code clones in context, In Proceedings of International Conference on Software Engineering, pp.762-766, 2007.

\bibitem{Al-Omari2012}	F. Al-Omari, I. Keivanloo, C. K. Roy, and J. Rilling, Detecting clones across microsoft .net programming languages, In Proceedings of Working Conference on Reverse Engineering, pp.405-414, 2012.

\bibitem{Al-Omari} F. Al-Omari, I. Keivanloo, C. K. Roy, and J. Rilling, Detecting clones across Microsoft .net programming languages, In Proceeding of Working Conference on Reverse Engineering, pp.405-414, 2012.

\bibitem{Anquetil} N. Anquetil and T. C. Lethbridge, Recovering software architecture from the names of source files, Journal of Software Maintenance: Research and Practice, 11(3),pp.201-221, 1999.

\bibitem{Antoniol 2012} G. Antoniol, G. Canfora, G. Casazza, A. De Lucia and E. Merlo, Recovering traceability links between code and documentation, In Proceedings of IEEE Transactions on Software Engineering, 28(10), pp.970-983, 2002.

\bibitem{Asaduzzaman2012} M. Asaduzzaman, C. K. Roy, and K. A. Schneider, VisCad: Flexible code clone analysis support for NiCad, In Proceedings of International Workshop on Software Clones, pp.77-78, 2011.

\bibitem{avetisyan} A. Avetisyan, S. Kurmangaleev, S. Sargsyan, M. Arutunian,
and A. Belevantsev. LLVM-based code clone detection framework. Computer Science and Information Technologies, pp.100-104, 2015.

\bibitem{Baker1995} B. Baker, On Finding Duplication and Near-Duplication in Large Software Systems, In Proceedings of Working Conference on Reverse Engineering, pp. 86-95, 1995.

\bibitem{Basit} H. Basit, D. Rajapakse, and S. Jarzabek, An empirical study on limits of clone unification using generics, In Proceedings of SEKE, pp.109-114, 2005.

\bibitem{Baxter1998} I. Baxter, A. Yahin, L. Moura and M. Anna, Clone Detection Using Abstract Syntax Trees, In Proceedings of Software Maintenance, pp.368-377, 1998.

\bibitem{CloneDR}I.D. Baxter, A. Quigley, L. Bier, M. Sant’Anna, L. Moura, and A. Yahin, CloneDR: clone detection and removal, In Proceedings of the 1st International Workshop on Soft Computing Applied to Software Engineering, pp.111-117, 1999.

\bibitem{Baxter} I. Baxter, A. Yahin, L. Moura, M. Sant’Anna, and L. Bier, Clone detection using abstract syntax trees, In Proceedings of International Conference on Software Maintenance, pp.368-377, 1998.	

\bibitem{Bazrafshan}S. Bazrafshan, and R. Koschke, An empirical study of clone removals, In Proceedings of International Conference Software Maintenance, pp.50-59, 2013.

\bibitem{Bellon} S. Bellon, R. Koschke, G. Antoniol, J. Krinke, and E. Merlo, Comparison and evaluation of clone detection tools, IEEE Transaction on Software Engineering, 33(9), pp.577-591, 2007.

\bibitem{Bettenburg} N. Bettenburg, W. Shang, W. Ibrahim, B. Adams, Y. Zou, and A. Hassan, An empirical study on inconsistent changes to code clones at the release level, Science of Computer Programming, 77(6), pp.760-776, 2012.

\bibitem{Biggerstaff} T. J. Biggerstaff, B. G. Mitbander, and D. Webster, Program understanding and the concept assignment problem, Communications of the ACM, 37(5):pp.72-83, 1994.

\bibitem{LDA} D. Blei, A. Ng, and M. Jordan, Latent dirichlet allocation, Journal of Machine Learning Research, pp.993-1022, 2003.

\bibitem{Bouktif} S. Bouktif, G. Antoniol, M. Neteler, and E. Merlo, A novel approach to optimize clone refactoring activity, In Proceedings of Genetic and Evolutionary Computation, pp.1885-1892, 2006.

\bibitem{Caprile} B. Caprile and P. Tonella, Nomen est omen: Analyzing the language of function identifiers, In Proceedings of the Sixth Working Conference on Reverse Engineering, pp.112-122, 1999.

\bibitem{Chatterji}	D. Chatterji, J. C. Carver, and N. A. Kraft, Cloning: The need to understand developer intent, In Proceedings of International Workshop on Software Clones, pp.14-15, 2013.

\bibitem{Cheng} H. Cheng, X. Yan, and J. Han, Mining Graph Patterns, In Frequent Pattern Mining, pp.307-338, 2014.

\bibitem{clcminer} X. Cheng, Z. Peng, L. Jiang, H. Zhong, H. Yu, and J. Zhao, CLCMiner: Detecting Cross-Language Clones without Intermediates. IEICE Trans, on Information and Systems, 100(2), pp.273-284, 2017.
\bibitem{nicad} J.R. Cordy and C. K. Roy, The NiCad clone detector, In Proceedings of Program Comprehension (ICPC), pp.219-220, 2011.

\bibitem{Cordy2003}	J. R. Cordy. Comprehending reality: Practical barriers to industrial adoption of software maintenance automation, In Proceedings of International Workshop on Program Comprehension, pp.196-206, 2003.

\bibitem{Cordy2011}	J. R. Cordy, Live scatterplots, In Proceedings of International Workshop on Software Clones, pp.79-80, 2011.

\bibitem{Sdang} S. Dang and S. A. Wani, Performance Evaluation of Clone Detection Tools, International Journal of Science and Research, 2015
					
\bibitem{Davis} I. Davis and M. Godfrey, Clone detection by exploiting assembler, In Proceedings of 4th International Workshop on Software Clones, pp.77-78, 2010.

\bibitem{Ferrante}J. Ferrante, K. J. Ottenstein, and J. D. Warren, The program dependence graph and its use in optimization, ACM Transactions on Programming Languages and Systems, 9(3), pp.319-349, 1987.

\bibitem{Gabel} M. Gabel, L Jiang, Zhendong SU, Scalable detection of semantic clones, In Proceedings of the International Conference on Software Engineering, pp.321-330, 2008.

\bibitem{akash2018} A. Ghosh and S. K. Kuttal, Semantic Code Clones: Can Source Code Comments Help?, IEEE Conference VL/HCC, 2018.

\bibitem{Gode} N. Göde, and K. Rainer, Studying clone evolution using incremental clone detection,  Journal of Software: Evolution and Process, 25(2), pp.165-192, 2013.

\bibitem{Griffiths} T. Griffiths and M. Steyvers, Finding scientific topics, In Proceedings of the National Academy of Sciences, pp.5228-5235, 2004.

\bibitem{Grinstead} C. M. Grinstead and J. L. Snell, Introduction to Probability, American Mathematical Society, Providence, RI, 2 edition, 1997.

\bibitem{Gu2016} Xiaodong Gu, Hongyu Zhang, Dongmei Zhang, and Sunghun Kim. 2016. Deep
API learning. In Proceedings of the 2016 24th ACM SIGSOFT International Symposium on Foundations of Software Engineering. ACM, 631–642.

\bibitem{Haiduc2010a} Sonia Haiduc, Jairo Aponte, and Andrian Marcus. 2010. Supporting program
comprehension with source code summarization. In Proceedings of the 32nd
ACM/IEEE International Conference on Software Engineering-Volume 2. ACM, 223–
226.

\bibitem{Haiduc2010b} Sonia Haiduc, Jairo Aponte, Laura Moreno, and Andrian Marcus. 2010. On the
use of automated text summarization techniques for summarizing source code.
In Reverse Engineering (WCRE), 2010 17th Working Conference on. IEEE, 35–44.

\bibitem{Henderson} TAD Henderson and A Podgurski, Sampling code clones from program dependence graphs with GRAPLE, In Proceedings of the 2nd International Workshop on Software Analytics, pp.47-53, 2016.

\bibitem{Higo} Y. Higo and S. Kusumoto, Code Clone Detection on Specialized PDGs with Heuristics, In Proceedings of Software Maintenance and Reengineering, pp.75-84,  2011.

\bibitem{Higo2011} Y. Higo, U. Yasushi, M. Nishino, and S. Kusumoto, Incremental code clone detection: A PDG-based approach, In Proceedings of Working Conference on Reverse Engineering, pp.3-12, 2011

\bibitem{Higo2009} Y. Higo and S. Kusumoto, Enhancing quality of code clone detection with program dependency graph, In Proceedings of Working Conference on Reverse Engineering, pp.315-316, 2009.

\bibitem{Higo13} Yoshiki Higo and Hiroaki Murakami and Shinji Kusumoto, Revisiting Capability of PDG-based Clone Detection, Technical Report, Graduate School of Information Science and Technology, Osaka University, 2013.

\bibitem{rafhoff} R. Hoffmann, J. Fogarty, and D. S. Weld, Assieme: finding and leveraging implicit references in a web search interface for programmers, In
Proceedings of the 20th annual ACM symposium on User interface software and
technology, pp.13–22, 2007.

\bibitem{hu2018} Xing Hu, Ge Li, Xin Xia, David Lo, and Zhi Jin. 2018. Deep code comment generation. In Proceedings of the 26th Conference on Program Comprehension, 200-210.

\bibitem{JAVASwing} 
Java Swing: https://docs.oracle.com/javase/javax/swing/package-summary.html

 \bibitem{JHD} JHotDraw: http://www.jhotdraw.org/

\bibitem{Lxiang} L. Jiang and Z. Su, Automatic mining of functionally equivalent
code fragments via random testing. In Proceedings of the eighteenth international
symposium on Software testing and analysis, pp.81–92, 2009.

\bibitem{Johnson}J. Johnson, Visualizing Textual Redundancy in Legacy Source, In Proceedings of CASCON, pp.171-183, 1994.

\bibitem{Howard1994} J. Howard Johnson, Visualizing textual redundancy in legacy source, In Proceedings of the conference of the Centre for Advanced Studies on Collaborative research, John Botsford, Ann Gawman, Morven Gentleman, Evelyn Kidd, Kelly Lyons, Jacob Slonim, and Howard Johnson (Eds.). IBM Press, 1994.

\bibitem{Kapser2006} C. Kapser and M. Godfrey, Supporting the Analysis of Clones in Software Systems: A Case Study. Journal of Software Maintenance and Evolution: Research and Practice , 18(2), pp.61-82, 2006.

\bibitem{Keivanloo} I. Keivanloo, C. K. Roy, and J. Rilling, SeByte: Scalable clone and similarity search for bytecode, Science of Computer Programming, 95, 2014

\bibitem{kim} H. Kim, Y. Jung, S. Kim, and K. Yi, MeCC: Memory comparison-based
clone detector, In Proceedings of the 33rd International Conference on Software
Engineering, pp.301–310, 2011.

\bibitem{Facoy2018} K. Kim, D. Kim, TF Bissyande, E. Choi, L.li, J. Klein, Y. Le Traon,  FaCoY–A Code-to-Code Search Engine, In Proceedings of the 40th International Conference on Software Engineering, 2018

\bibitem{Komondoor} R. Komondoor and S. Horwitz, Using Slicing to Identify Duplication in Source Code, In Proceedings of International static analysis symposium, pp.40-56, 2001.

\bibitem{kraft} N. A. Kraft, B. W. Bonds, and R. K. Smith, Cross-language Clone Detection, In Proceedings of SEKE, pp.54-59, 2008.

\bibitem{Krinke} J. Krinke, Identifying similar code with program dependence graphs. In Proceedings of Working Conference on Reverse Engineering, pp.301-309, 2001. 

\bibitem{Kuhn} A. Kuhn, S. Ducasse, and T. Gˆırba, Semantic clustering: Identifying topics in source code, Information and Software Technology, 49(3), 2006. 

\bibitem{shihan} S. Li, X. Xiao, B. Bassett, T. Xie, and Nikolai Tillmann, Measuring Code Behavioral Similarity for Programming and Software Engineering
Education, In Proceedings of the 38th International Conference on Software
Engineering Companion, pp.501–510, 2016.

\bibitem{MCIdiff} Y. Lin, Z. Xing, Y. Xue, Y. Liu, X. Peng, J. Sun, and W. Zhao, Detecting differences across multiple instances of code clones, In Proceedings of International Conference on Software Engineering, pp.164-174, 2014.

\bibitem{dejavu} Lopes, Cristina V., Petr Maj, Pedro Martins, Vaibhav Saini, Di Yang, Jakub Zitny, Hitesh Sajnani, and Jan Vitek, DéjàVu: a map of code duplicates on GitHub, In Proceedings of the ACM on Programming Languages 1, OOPSLA, pp.84, 2017

\bibitem{Loyola2017} Pablo Loyola, Edison Marrese-Taylor, and Yutaka Matsuo. 2017. A Neural Architecture for Generating Natural Language Descriptions from Source Code
Changes. arXiv preprint arXiv:1704.04856 (2017).

\bibitem{Girish} G. Maskeri, S Sarkar and K Heafield, Mining business topics in source code using latent dirichlet allocation, In Proceedings of 1st India software engineering conference, pp.113-120, 2008.

\bibitem{Mayrand1996} J. Mayrand, C. Leblanc and E. Merlo, Experiment on the Automatic Detection of Function Clones in a Software System Using Metrics, In Proceeding of ICSM, pp.244-253, 1996Measuring Code Behavioral Similarity for Programming and Software Engineering
Education.

\bibitem{McBurney2014} Paul W McBurney and Collin McMillan. 2014. Automatic documentation generation via source code summarization of method context. In Proceedings of the
22nd International Conference on Program Comprehension. ACM, 279–290.

\bibitem{Moreno2013} Laura Moreno, Jairo Aponte, Giriprasad Sridhara, Andrian Marcus, Lori Pollock,
and K Vijay-Shanker. 2013. Automatic generation of natural language summaries
for java classes. In Program Comprehension (ICPC), 2013 IEEE 21st International Conference on. IEEE, 23–32.

\bibitem{Nakakoji} K. Nakakoji, Y. Yamamoto, Y. Nishinaka, Kouichi Kishida, and Y. Ye, Evolution Patterns of Open-Source Software Systems and Communities, In Proceedings of the International Workshop on Principles of Software Evolution, pp.76-85, 2002.

\bibitem{Oezbek} C. Oezbek and L. Prechelt, JTourBus: Simplifying Program Understanding by Documentation that Provides Tours Through the Source Code, In Proceedings of IEEE International Conference on Software Maintenance, pp.64-73, 2007.

\bibitem{Pham} N. H. Pham, H. A. Nguyen, T. T. Nguyen, J. M. Al-Kofahi, and T. N. Nguyen, Complete and accurate clone detection in graph-based models, In Proceedings of International Conference on Software Engineering, pp.276-286, 2009

\bibitem{PYGUI} PyGUI: http://www.cosc.canterbury.ac.nz/greg.ewing/pythongui/version/
Doc/index.html

\bibitem{exp} https://docs.python.org/3/tutorial/errors.html

\bibitem{quality} C. K. Roy, J. R. Cordy, and R. Koschke, Comparison and evaluation of code clone detection techniques and tools: A qualitative approach, Science of Computer Programming, 74(7), 2009.

\bibitem{Roy2007} C. K. Roy and J. R. Cordy, A survey on software clone detection research, Technical Report TR 2007-541, Queens University, 2007.

\bibitem{Roy2014} C.K. Roy, M.F. Zibran, and R. Koschke, The vision of software clone management: Past, present, and future (Keynote paper), In Proceedings of IEEE Software Maintenance, Reengineering and Reverse Engineering, pp.18-33, 2014.

\bibitem{Seidl} D. Seidl, B. Hummel and E. Juergens, Quality Analysis of Source Code comments, In Proceedings of International Conference on Program Comprehension, pp.43-60, 2013.

\bibitem{survey} A. Sheneamer and J. Kalita, Article: A Survey of Software Clone Detection Techniques, International Journal of Computer Applications, 137(10) 2016.

\bibitem{Podgurski} G. Shu, B.Sun, T.A.D. Henderson and A. Podgurski, JavaPDG: A New Platform for Program Dependence Analysis, In Proceedings of International Conference on Software Testing, Verification and Validation, pp.408-415, 2013.

\bibitem{Sirres} R. Sirres, T. F. Bissyandé, D. Kim, D. Lo, J. Klein,
K. Kim, and Y. L. Traon, Augmenting and Structuring User Queries to Support Efficient Free-Form Code Search, In Proceedings of Empirical Software Engineering, 23(5), pp.2622–2654, 2018.

\bibitem{Souza} S. C. B. de Souza, N. Anquetil, and K. M. de Oliveira, A Study of the Documentation Essential to Software Maintenance, In Proceedings of the 23rd annual international conference on Design of communication: documenting \& designing for pervasive information, pp.68-75, 2005.

\bibitem{Sridhara2010} Giriprasad Sridhara, Emily Hill, Divya Muppaneni, Lori Pollock, and K VijayShanker. 2010. Towards automatically generating summary comments for java
methods. In Proceedings of the IEEE/ACM international conference on Automated
software engineering. ACM, 43–52.

%\bibitem{Sridhara2010} Giriprasad Sridhara, Emily Hill, Divya Muppaneni, Lori Pollock, and K VijayShanker. 2010. Towards automatically generating summary comments for java methods. In Proceedings of the IEEE/ACM international conference on Automated software engineering. ACM, 43–52.

\bibitem{Iyer2016} Srinivasan Iyer, Ioannis Konstas, Alvin Cheung, and Luke Zettlemoyer. 2016.
Summarizing Source Code using a Neural Attention Model.. In ACL (1).

\bibitem{KTStolee} K. T. Stolee, S. Elbaum, and Daniel Dobos, Solving the Search
for Source Code, ACM Transactions on Software Engineering Methodology, 23(3), pp.26, 2014

\bibitem{fhsu} F. H. Su, J. Bell, K. Harvey, S. Sethumadhavan, G.
Kaiser, and T. Jebara, Code Relatives: Detecting Similarly Behaving
Software, In Proceedings of the 2016 24th ACM SIGSOFT International Symposium
on Foundations of Software Engineering (FSE 2016), pp.702–714, 2016.

\bibitem{duplicate} M. Sudhamani and L. Rangarajan, Duplicate Code Detection using Control Statements, International Journal of Computer Applications Technology and Research, 4(10), 2015

\bibitem{Tenny} T. Tenny, Program Readability: Procedures Versus Comments, IEEE Transactions of Software Engineering, 14(9), pp.1271-1279, 1988.

\bibitem{Thompson} S. K. Thompson. Sampling. John Wiley and Sons, New York, 2 edition, 2002.

\bibitem{LICCA2018} T. Vislavski, G. Rakic, Z and N Budimac, LICCA: A tool for cross-language clone detection, 2018 IEEE 25th International Conference on Software Analysis, Evolution and Reengineering, pp.512-516, 2018

\bibitem{Wang2016} Song Wang, Taiyue Liu, and Lin Tan. 2016. Automatically learning semantic
features for defect prediction. In Proceedings of the 38th International Conference
on Software Engineering. ACM, 297–308.

\bibitem{Wilde} N. Wilde, M. Buckellew, H. Page, V. Rajlich, and L. Pounds, A comparison of methods for locating features in legacy software, Journal of Systems and Software, 65(2), pp.105-114, 2003.

\bibitem{white} M. White, M. Tufano,C.Vendome, and D. Poshyvanyk, Deep learning code fragments for code clone detection, In Proceedings of the 31st IEEE/ACM International Conference on Automated Software Engineering, pp.87-98, 2016

\bibitem{White2016} Martin White, Michele Tufano, Christopher Vendome, and Denys Poshyvanyk.
2016. Deep learning code fragments for code clone detection. In Proceedings of
the 31st IEEE/ACM International Conference on Automated Software Engineering.
ACM, 87–98.

\bibitem{Woodfield} S. N. Woodfield, H. E. Dunsmore, and V. Y. Shen, The effect of modularization and comments on program comprehension, In Proceedings of International Conference on Software Engineering, pp.215-223, 1981.

\bibitem{Saini2018} Vaibhav Saini, Farima Farmahini farahani, Yadong Lu, Pierre Baldi, and Cristina V. Lopes, Oreo: detection of clones in the twilight zone, In Proceedings of European Software Engineering Conference and Symposium on the Foundations of Software Engineering, pp 354-365, 2018.

\bibitem{Wang2018} Wang, Pengcheng, et al., CCAligner: a token based large-gap clone detector, Proceedings of the 40th International Conference on Software Engineering (ICSE). ACM, 2018.

\bibitem{Sajnani2016} Sajnani, Hitesh, et al., SourcererCC: scaling code clone detection to big-code, In Proceedings of International Conference on Software Engineering, 2016.

\bibitem{Roy2008} Roy, Chanchal K., and James R. Cordy, NICAD: Accurate detection of near-miss intentional clones using flexible pretty-printing and code normalization, 16th IEEE international conference on program comprehension (ICPC), 2008.

\bibitem{Hong2010} Liangjie Hong and Brian D. Davison, Empirical study of topic modeling in Twitter, In Proceedings of the First Workshop on Social Media Analytics, pp 80-88, 2010. 

\bibitem{wikipop} https://en.wikipedia.org/wiki/Latent\_Dirichlet\_allocation

\bibitem{Bellon2007} S. Bellon, R. Koschke, G. Antoniol, J. Krinke and E. Merlo, "Comparison and Evaluation of Clone Detection Tools," in IEEE Transactions on Software Engineering, vol. 33, no. 9, pp. 577-591, Sept. 2007.




\end{thebibliography}

==> discussions.tex <==
\section{Discussions}

Table \ref{jhotdraw} summarizes the number of clone sets reported, the recall, and the precision of LDA (with the different ways) and PDG (without and with probability). Our results show that we can utilize comments for detecting the code clones. When we applied the LDA technique to the comments, we found that for the topic size of 200, the precision and accuracy both stayed constant despite the fact that recall and precision varied with the number of source files in the corpus, i.e. the size of the package. Based on our results, LDA performed somewhat better than PDG. 

\begin{figure}
\centerline{\includegraphics[width=0.5\textwidth]{images/lang.png}}
\caption{Comparison of languages}
\label{lang}
\end{figure}


We recommend the use of a hybrid technique, i.e. utilizing both LDA and PDG to find the semantic clones. After collecting clone sets based on the similarity indices, we created a superset containing all those files. The superset contained unique file names. In our case we found 40-50 common files. This superset can be used as input for PDG based techniques like GRAPLE to detect function level clones. This will help in utilizing code as well as the comments of a program to find unique sets of clones. Processing all clone dependencies for even moderately sized programs is impractical. As noted by \cite{Henderson}, for programs with 70 KLOC, around 10 million clones were detected before the space was exhausted.  LDA can be utilized to generate the clone sets at file level and then PDG based techniques can be applied on these selected clone sets to find the function level clones. 

Further, finding clones in multi-languages is still an open research problem. We believe that comments can help in supporting interoperability across several programming languages. Figure \ref{lang} shows two examples, one from java code (in jHotDraw package) and another from python (python documentation \cite{exp}). Both are examples of classes that create an instance of exception with the arguments' name (the name of the element where error is located) and the message (describing what went wrong). Utilizing comments in this case can help in finding both types of programs. Still, we need to empirically evaluate whether we can harness comments for detecting clones across languages.

The false positives and false negatives might have some repercussions in the detection mechanism. However, it still satisfies all the Research Questions. Consider, the case studies where LDA found a clone and PDG didn't. In such a scenario, the hybrid approach can be used, at first apply LDA on the source files to generate LDA clone sets which then can be used as an input for the GRAPLE to detect clones at a function level. Additionally, the logic upholds even when LDA misses a source file but GRAPLE identifies it as a clone set. However, when both of them miss out a clone set as mentioned in the \ref{results} sections, it would be nearly impossible to find that clone set. However, one approach would be to use transitive property to infer a clone set. Though, our approach didn't detect any such case, a theoretical example would be, if LDA detected a clone set [CS\_1, CS\_2] and PDG detected a clone set [CS\_3, CS\_2], which would mean [CS\_1, CS\_2, CS\_3] considering the exact clone set exists in the ground truth.

%Moreover, we can use GRAPLE without selection probabilities instead, since correlation between the two clone sets (GRAPLE with Pr and GRAPLE without Pr) seen before is high, so the performance will be approximately same without compromising time.


==> intro.tex <==
\section{Introduction}
\label{sec:intro}

``Don't reinvent the wheel, just realign it''. A common practice for programmers to increase their productivity is copying an existing piece of code and changing it to suit a new context or problem.  This reuse mechanism promotes large fragments of duplicate or near-duplicate  code in the code base \cite{Howard1994}. These duplicates are called code clones. Research shows that about 7\% to 23\% of software systems contain duplicated codes \cite{Baker1995, Baxter1998, Kapser2006, Mayrand1996}. In many cases, code clones are also generated unintentionally by programmers as they are working on similar programming tasks, overcoming limitations of programming languages, following coding conventions of an organization, or using design patterns \cite{Roy2007}. To support reuse, various code detection techniques have been utilized to find similarities between the code fragments \cite{Roy2014}. These code detection techniques are based on Tokens  \cite{Bouktif,Adar, Bettenburg}, Abstract Syntax Tree \cite{Al-Omari2012,Bazrafshan} and Program Dependency Graph \cite{Chatterji, Cordy2003, Henderson}. 

One of the most challenging types of clones to find is semantic clones - code fragments that are functionally similar but may be syntactically different. Techniques based on Program Dependency Graph are the most notable mechanisms to detect semantic code clones\cite{Henderson}. Since PDG helps abstract many arbitrary syntactic decisions that a programmer made while constructing a function, they serve as the best fit for finding semantic code clones \cite{Gabel}. However, PDG-based techniques are computationally expensive, as they require resource-intensive operations to detect the clones \cite{Bellon}.

%It calculates the dependency of two clones based on the corresponding occurrence of subgraphs in a graph set.

\begin{figure*}[h]
\centerline{\includegraphics[width=\textwidth]{images/fours.png}}
\caption{DrawApplet, NetApplet, SVGApplet and PertApplet source files in a clone set found by LDA in JHotDraw package.}
\label{fours}
\end{figure*} 

Current clone detection techniques are solely based on the source code and ignore the source code comments. From a program comprehension point of view, comments carry important domain knowledge and assist programmers in understanding the software system\cite{Johnson, Seidl, Oezbek, Tenny, Woodfield}. Further, a significant amount of source code in software systems consists of comments   \cite{Souza}. Hence, a major part of the program is ignored while detecting the clones.

%Further, it is known that code comments help in better code understanding while developing or using the code for source code understanding than the source code itself  \cite{Tenny,Woodfield}. 

 The prime reason for clone detection techniques to ignore code comments is the ambiguity of the English language. For example, the three words ``Hotel,'' ``Motel,'' and ``Inn'' are under the same umbrella of the topic of ``a place to stay.'' For humans, it is easy to comprehend the similarity or difference between the words or topics, but a machine may treat the words differently. However, with the recent advancement in topic modeling techniques, we are able to make more accurate predictions using machine learning and natural language processing tools. One of the most versatile topic modeling techniques is Latent Dirichlet Allocation (LDA), which has been used extensively for text mining the hidden topic patterns.
 
In this paper, we investigated: 
\begin{itemize}
  \item \textbf{RQ1:} Does the use of comments help in detecting semantic clones in the code base?  
  \item \textbf{RQ2:} Does a PDG based technique, which just uses code for detection of semantic clones, perform equivalently to an LDA based technique, which uses comments?
  \item \textbf{RQ3:} Does our evaluation technique performs equally across multiple languages?

\end{itemize}

% To answer our research questions, we analyzed the open source software JHotDraw\cite{JHD}. To detect clone sets in the JHotDraw package, we analyzed code by using the PDG-based tool GRAPLE \cite{Henderson}, and we  analyzed comments using LDA. 
To answer our first 2 research questions, we analyzed the open source software JHotDraw. To detect clone sets in the JHotDraw package, we analyzed code by using the PDG-based tool GRAPLE \cite{Henderson}, and we analyzed comments using LDA. To answer our third research question we analyzed two popular graphics packages, PyGUI and Java Swing. We also tried to compare between clone sets generated by GRAPLE and LDA using Java NIO and JFreeChart, to underpin our hypothesis.

310 java source files with 27kLOC. 

==> motivation.tex <==
\section{Motivation}
\label{sec:motiv}


% \begin{figure}
% \centerline{\includegraphics[width=0.5\textwidth]{images/lang.png}}
% \caption{Sample code example from java and python with same functionality \cite{JHD, PYGUI}.}.
% \label{lang}
% \vspace{-20pt}
% \end{figure}

In software engineering, detecting similar code fragments beyond syntactical similarities has been a conundrum. The challenge lies in developing a unified approach to detecting semantically similar code fragments in a single or across multiple languages. This section motivates the cause of the research. 

\textbf{\emph{Detecting code comments within a same platform:}} The state-of-the-art clone detection techniques focus on generating intermediate representations.These approaches \cite{LICCA2018, clcminer}, rely on programs that yield the same outputs using dynamic code similarity detection \cite{Lxiang, shihan, kim}, and identifying similar behaviours of different programs by comparing instruction-level execution \cite{fhsu}. These approaches are precise but are not scalable and have limitations for practical usage. Nonetheless, none these approaches have considered code comments for identifying similar code fragments. This paper explores the feasibility of using code comments as a parameter for clone detection. A sample output of our approach would be Fig. \ref{fours} which depicts four source files which were found by both PDG and LDA as a clones set. All of these four classes extend the JApplet class with little variation in the try-catch block. However, the functionality of all four of the classes are the same. A snippet of these comments are shown, where it is clearly stated that it overrides the JApplet functionalities by using the \texttt{getParameter} function. Thus, our approach detects clones as precisely and efficiently as the other state-of-the-art detection techniques. 

\begin{figure}
\centerline{\includegraphics[width=0.5\textwidth]{images/cross.png}}
\caption{Sample code example from java and python with same functionality}.
\label{cross}
\end{figure}

\textbf{\emph{Detecting code comments across platforms:}} Fig. \ref{cross} depicts two source files, Java and Python. Here, it can be observed that both the files have similar structure with some exceptions in the arguments, but functionally perform the same task. The Python code fragment calls the Error class which handles all the exceptions in Python. Here, this piece of code handles only exceptions raised during exiting an event loop action. The Java code fragment shows a constructor of \texttt{ExpandVetoException Class} which extends the \texttt{Exception Class} of Java. Here, it takes two arguments \texttt{event} and \texttt{message} to call the constructor of the \texttt{Exception class} which is similar to the behaviour of the Python code. In addition, in cases where most state-of-the-art approaches are inept, our approach works adequately in detecting clone sets.

\begin{figure*}l
\centerline{\includegraphics[width = 15cm]{images/motiv.png}}
\caption{Code retrieved from internet}.
\label{expcodes}
\end{figure*}

\textbf{\emph{We provide a scenario to better understand the cause of the research:}} Consider a scenario: Emily is a computer enthusiast high school student who wants to learn the art of programming. She starts with writing some Java code, which will also help her solve assignments on the factorial of a number. With her limited l, she experiments with the code, and gets stuck after writing some part of it (Fig. ~\ref{expcodes}[1]). However, as the deadline approaches the time to experiment with code diminishes. Ergo, Emily goes online to search for the remaining part of code. She visits multiple websites but none of the online code bases match with the logic she upholds. In such scenarios, our detection mechanism can search with a matching logic, which is done by the text mining technique, Latent Dirichlet Allocation (LDA). One can find the types of code as depicted in Fig. ~\ref{expcodes}[2,3,4] when searched for on online code repositories. The best case match for Emily's code would be Fig ~\ref{expcodes} [2]. It is quite obvious that a factorial of a number can be written in multiple ways, using \texttt{for loop}, ternary operations or even recursion. In Emily's case, she used a sophisticated recursion logic. Of course using recursion to find factorial of a number is quite common - we used a simple scenario just to explain the problem, however, in large complex programs, a part of a code that matches with the written logic is extremely difficult to find. This problem can be solved easily by using the same text mining technique.

\begin{figure*}
\centerline{\includegraphics[width = 15cm]{images/fragments.png}}
\caption{Code Fragments extracted}.
\centerline{\includegraphics[width = 15cm]{images/pdgs.png}}
\caption{Program Dependence Graphs of the Fragments}.
\label{frag_pdg}
\end{figure*}

\textbf{\emph{To understand the detection mechanism behind LDA and PDG we considered a simple example Fig. \ref{lda_model_motiv}:}} The basic steps required to detect similar code fragments can be broken down to primary 3 steps.

\begin{enumerate}
  \item Detect pair of clones.
  \item Remove subsumed code fragments.
  \item Combine pairs of clones using transitive property to a larger set.
\end{enumerate}

\textbf{\emph{Program Dependence Graph:}} The detection of clone pairs can be easily done by generating a program dependence graph (PDG). We look for isomorphic subgraphs, obtained by backward and forward slicing. Fig. \ref{frag_pdg} shows two code fragments extracted from \textit{bison} and their relevant PDGs. The idea is to start with a backward slicing in a lock step and add predecessor to one slice only if there exists a corresponding matching predecessor in the other PDG. Forward slicing is used in case of a pair of matching loop or if-then-else. Nodes 4(a) and 4(b) are a match, and we backward slice along their inwards control-dependence edges to node 1. However, node 1 of both the graphs do not match, so we move onto the next inward edges 3(a), 4(a), 5(a) and 7 for the first PDG and 3(b), 4(b), 5(b) for the second PDG. Nodes 3(a) and 3(b) match and 5(a)-5(b) match so these nodes get added to the partial slices. As we slice backward from node 3(a) and 3(b) we find nodes 2(a) and 2(b) which match as well and thus get added to the partial slice. Now, 2(a) and 2(b) are represented with \textit{if} predicate, so we use forward slicing and reach node 2(a) and 2(b), since they are already added to the partial slice, so they are not considered. The last step in the slicing process is to move onto node 5(a) and 5(b), slicing backward we reach to node 1 (which is not a match). We represented these two partial slices with the ``++" sign in the code fragments. As one can observe, traversing through the graphs to find isomorphic subgraphs can be extremely demanding, thus our approach focuses on LDA - more efficient approach.

\begin{figure*}
\centerline{\includegraphics[width = 15cm]{images/LDAmodel2.png}}
\caption{LDA model with comments extracted}.
\label{lda_model_motiv}
\end{figure*}

\textbf{\emph{Latent Dirichlet Allocation:}} Fig. \ref{lda_model_motiv}, shows a demonstration of how LDA works. Two code comments have been extracted from two source files, namely from XMLParseException and XMLException. Each of these source files has been labelled with multiple topics. However, Fig. \ref{lda_model_motiv}, shows labelling of each file with two most relevant topics. The bold arrows depict the highest relevance between the comments and a topic, whereas the dashed arrows depict the next best relevance between them. Both the source files have the highest relevance with Topic 3; the highlighted words indicates the occurrence of each word in respect to their topic. The detection mechanism implemented by LDA is much faster and more efficient in comparison to PDG. 



==> old-conclusion.tex <==
This is the first study to investigate the realm of code comments to detect code clones. Our results revealed:
\begin{enumerate}
 
\item \textit{RQ1: Utilizing code comments:} Our findings support that code comments can be utilized in the detection of clone sets using topic modeling techniques, and are equivalent to sophisticated PDG-based techniques. The ability of LDA to detect clones depended on the quality of comments, while PDG’s ability to detect clones depended on the constraints applied to the tool. The vague/incomplete comments produced a large number of false positives.
\item \textit{RQ2: Hybrid Approach:} Both LDA and PDG techniques can be applied for detecting clones using a hybrid approach: First, utilize comments with the topic modeling techniques (LDA) to detect clone sets at the file level, as this process is less resource-intensive. Second, utilize code by applying PDG-based code detection techniques at the function level, as they are more rigorous mechanisms.
\item \textit{RQ3: Across Languages:} Our results show that quality comments can be utilized to find clones across programming languages to an extent.

\end{enumerate}
